Efficient learning of smooth probability functions from Bernoulli tests with guarantees

We study the fundamental problem of learning an unknown, smooth probability function via pointwise Bernoulli tests. We provide a scalable algorithm for efficiently solving this problem with rigorous guarantees. In particular, we prove the convergence rate of our posterior update rule to the true probability function in L2-norm. Moreover, we allow the Bernoulli tests to depend on contextual features and provide a modified inference engine with provable guarantees for this novel setting. Numerical results show that the empirical convergence rates match the theory, and illustrate the superiority of our approach in handling contextual features over the state-of-the-art.

==> commands.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% if you need to pass options to natbib, use, e.g.:
% \PassOptionsToPackage{numbers, compress}{natbib}
% before loading nips_2017
%
% to avoid loading the natbib package, add option nonatbib:
%\usepackage[nonatbib]{nips_2018}

%\usepackage{nips_2018}

%\usepackage[square,sort]{natbib}
%\usepackage[authoryear,round,longnamesfirst]{natbib}

% to compile a camera-ready version, add the [final] option, e.g.:
% \usepackage[final]{nips_2017}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The following packages will be automatically loaded:
% amsmath, amssymb, natbib, graphicx, url, algorithm2e

\usepackage[lined, boxed, ruled, commentsnumbered]{algorithm2e}
%, noend

\usepackage{times}

\usepackage{hyperref}
\usepackage{mathtools}
\usepackage{multirow,color,graphicx}
\usepackage{subfloat}
\usepackage{xfrac,amsfonts,amsbsy}
\usepackage[titletoc]{appendix}
\usepackage{xspace}
\usepackage{savesym,verbatim}
\usepackage[titletoc]{appendix}
\usepackage{paralist}
\usepackage{subscript}
\usepackage{tikz}

\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{float}
\usepackage{enumitem}
\usepackage{caption}
\usepackage{subcaption}

% \usepackage[tight]{subfigure}
\usepackage{amsthm}

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{remark}{Remark}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother
%\newcounter{copyrightbox}
%\setlength{\abovecaptionskip}{2pt}
%\setlength{\belowcaptionskip}{2pt}
%\setlength{\intextsep}{3pt} % between float and text, float in "h" here
%\setlength{\dblfloatsep}{0.15 \baselineskip plus 3pt minus 2pt} % between two floats
%\setlength{\dbltextfloatsep}{0.15 \baselineskip plus 3pt minus 2pt} % between float and text, float on "t" top or "b" botton
%\setlength\floatsep{0.15 \baselineskip plus 3pt minus 2pt} % between two floats
%\setlength\textfloatsep{0.15 \baselineskip plus 3pt minus 2pt} % float on top or botton

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{titlesec}
\titlespacing*{\section}
{0pt}{2.ex plus 1ex minus .2ex}{1.0ex plus .2ex}
\titlespacing*{\subsection}
{0pt}{1.0ex plus 1ex minus .2ex}{1.0ex plus .2ex}

\setlength{\parskip}{2pt plus1.5mm minus1.5mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NIPS'16
%\usepackage{titlesec}
%\titlespacing*{\section}
%{0pt}{2.ex plus 1ex minus .2ex}{1.0ex plus .2ex}
%\titlespacing*{\subsection}
%{0pt}{1.0ex plus 1ex minus .2ex}{1.0ex plus .2ex}
%%\setlength{\parskip}{0.1cm plus2mm minus2mm}
%
%\setlength{\parskip}{2pt plus1.5mm minus1.5mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\citetnew}[1]{\citeauthor{#1} (\citeyear{#1})}
%\newcommand{\citet}[1]{\citeauthor{#1} (\citeyear{#1})}

% argmin and argmax
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\renewcommand{\algorithmcfname}{Algorithm}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}

\newcommand{\pushline}{\Indp}% Indent
\newcommand{\popline}{\Indm\dosemic}% Undent


\newcommand{\indfunc}{\ensuremath{\mathbf{1}}}

\newcommand{\bigObound}{\ensuremath{\mathcal{O}}}
\newcommand{\smallObound}{\ensuremath{o}}
\newcommand{\Thetabound}{\ensuremath{\Theta}}
\newcommand{\Omegabound}{\ensuremath{\Omega}}

\newcommand{\full}{\textsc{Full}\xspace}
\newcommand{\anyalg}{\textsc{Alg}\xspace}
\newcommand{\hedge}{\textsc{Hedge}\xspace}
\newcommand{\expthree}{\textsc{EXP3}\xspace}
\newcommand{\expfour}{\textsc{EXP4}\xspace}
%%%%
\newcommand{\algoshort}{\textsc{LExp}\xspace}
\newcommand{\algo}{\textsc{LearnExp}\xspace}
\newcommand{\generalalgo}{\textsc{Algo}\xspace}
%%%%
\newcommand{\adv}{\textsc{Adv}\xspace}
\newcommand{\expert}{\textsc{Exp}\xspace}
\newcommand{\experts}{\textsc{Exps}\xspace}
\newcommand{\num}{\ensuremath{N}}
\newcommand{\numinterests}{\ensuremath{M}}

\newcommand{\actionSet}{\ensuremath{\mathcal{A}}}
\newcommand{\action}{\ensuremath{a}}

\newcommand{\contextSet}{\ensuremath{\mathcal{X}}}
\newcommand{\context}{\ensuremath{x}}
\newcommand{\interest}{\ensuremath{I}}

\newcommand{\price}{\ensuremath{c}}
\newcommand{\priceSet}{\ensuremath{C}}
%\newcommand{\cost}{\ensuremath{c}}

\newcommand{\outcomeSet}{\ensuremath{\mathcal{Y}}}
\newcommand{\outcome}{\ensuremath{y}}

\newcommand{\gradientSet}{\ensuremath{\mathcal{Z}}}
\newcommand{\gradient}{\ensuremath{z}}

%\newcommand{\paramSet}{\ensuremath{\boldsymbol{\theta}}}
%\newcommand{\param}{\ensuremath{\theta}}
\newcommand{\paramSet}{\ensuremath{S}}
\newcommand{\param}{\ensuremath{w}}

\newcommand{\learningRate}{\ensuremath{\eta}}
\newcommand{\auxl}{\ensuremath{\alpha}}
\newcommand{\regretRate}{\ensuremath{\beta}}
\newcommand{\smoothRate}{\ensuremath{\alpha}}

\newcommand{\rewardFunc}{\ensuremath{\mathcal{R}}}
\newcommand{\lossFunc}{\ensuremath{\mathcal{L}}}
\newcommand{\feedbackFunc}{\ensuremath{\mathcal{F}}}
\newcommand{\reward}{\ensuremath{r}}
\newcommand{\loss}{\ensuremath{l}}
\newcommand{\feedback}{\ensuremath{f}}

\newcommand{\val}{\ensuremath{V}}
\newcommand{\Time}{\ensuremath{T}}
%\newcommand{\omdT}{\ensuremath{\boldsymbol{\tau}}}
\newcommand{\omdT}{\ensuremath{T}}

\newcommand{\rewardmax}{\ensuremath{r_{max}}}
\newcommand{\lossmax}{\ensuremath{l_{max}}}

\newcommand{\sequence}{\ensuremath{\mathcal{D}}}
%\newcommand{\sequencelen}{\ensuremath{\ensuremath{\tau}}}
\newcommand{\sequencelen}{\ensuremath{|\mathcal{D}|}}

\newcommand{\blocksz}{\ensuremath{B}}

\newcommand{\historySet}{\ensuremath{\mathcal{H}}}
\newcommand{\history}{\ensuremath{h}}

\newcommand{\regretext}{\textsc{RegExternal}\xspace}
\newcommand{\regretbexp}{\textsc{RegBExp}\xspace}
\newcommand{\regret}{\textsc{Reg}\xspace}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\corral}{\textsc{Corral}\xspace}

%\newcommand{\regret}{\textsc{Regret}\xspace}

\newcommand{\task}{\ensuremath{v}}
\newcommand{\tasks}{\ensuremath{\mathcal{V}}}
\newcommand\inner[2]{\langle #1, #2 \rangle}
\newcommand{\round}[1]{\left(#1\right)}
\newcommand{\brace}[1]{\left\{#1\right\}}
\newcommand{\feasibleset}{\mathcal{W}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\adish}[1]{{\textcolor{red}{{\bf AS:} #1}}}
%\newcommand{\hamed}[1]{{\textcolor{green}{{\bf HH:} #1}}}
%\newcommand{\ak}[1]{{\textcolor{red}{{\bf AK:} #1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EXTRA

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> experimental_details.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental details}

\subsection{Synthetic examples}\label{sec:experiments-synthetic-detail}

We present here the functions that have been used for the synthetic experiments, and the posterior means generated by algorithm~\ref{algo-static-setting} (Figure~\ref{fig:synthetic-functions}). For the 1D case, we also observe the approximated means for the various kernel we used. For the wide kernel with width $\Delta_1$ (in green), we observe that the approximation is too smooth an cannot model function we high slopes. This explains the saturation of the approximation error observe on Figure~\ref{fig:1D_static}. For the sharp kernel with width $\Delta_2$ (in red), the approximated mean is highly non-smooth, and thus hardly fits the target function.

\begin{figure*}[h!]
	\begin{center}
		\begin{subfigure}[t]{0.4\textwidth}
			\includegraphics[scale=0.2]{fig/static-1d-synthetic-belief.png}
			\caption{1D static setting: $f(x) = \frac{1}{8}\mathcal{B}(x;7,3) + \frac{1}{6}\mathcal{B}(x;3,7) + 0.2$ where $\mathcal{B}(x;\alpha,\beta)$ is the Beta probability distribution function with parameters $\alpha, \beta$.}
			\label{fig:convergence-rate-1d-static}
		\end{subfigure} 
		\hspace{6mm}
		\begin{subfigure}[t]{0.4\textwidth}
			\includegraphics[scale=0.2]{fig/static-2d-synthetic-belief.png}
			\caption{2D static setting: $f(x) = \mathcal{N}(x;(0.75, 0.75)^T,\sigma \cdot \textbf{I}) + \mathcal{N}(x;(0.6, 0.3)^T,\sigma \cdot \textbf{I})  + \mathcal{N}(x;(0.25, 0.6)^T,\sigma\cdot \textbf{I})$ where $\sigma=0.025$ and $\mathcal{N}(x;\mu,\Sigma)$ is the Normal probability distribution function with mean $\mu$ and covariance matrix, $\Sigma$.}
		\end{subfigure}
	\caption{Synthetic functions that have been generated for the experiments. The plots also show the mean posterior estimates $\mathbb{E}[\tilde{\func}(x|\mathcal{S})]$ generated by Algorithm~\ref{algo-static-setting}.}
		\label{fig:synthetic-functions}
	\end{center}
\end{figure*}



\subsection{A real-world application: Extended stroke rehabilitation case study}\label{sec.experiments-realworld-detail}

Note that \cite{goetschalckx2011continuous} studied this problem through a synthetic simulation for a particular scenario where they modeled fatigue as a binary variable (i.e. the patient is either fatigued or not). Inspired by their experiment, we devised a numerical setup in which our aim is to accurately assess patients' physical capabilities, i.e. their success rate, across a space of difficulty levels of an hypothetical rehabilitation device.

We assume that there are $Z \in \mathbb{N}$ different levels of fatigue $\{z_i\}_{i=1,...,Z}$, each decreasing the probability of success by a certain factor. Let $f_i$ denote the success probability function for fatigue level $i$, where $f_0$ is the non fatigue state ($z_0$) and $f_Z$ the highest fatigue level. For instance, $f_1(x)$ is the probability of success at fatigue level 1 for exercise difficulty level $x$. We further assume that success probability decreases linearly with difficulty of the exercise. 

Without loss of generality, we consider $\func_Z$ (highest level of fatigue) as the base function and all other functions $\func_{0, ..., Z-1}$ are increasing transformations of the form $(1 - B_i)\func_Z + B_i$. Precisely for this experiment, we take $Z = 5$ and $B_0 = 0.5$, $B_1 = 0.4$, $B_2 = 0.3$, $B_3 = 0.2$, $B_4 = 0.1$ and $B_5 = 0$. We define $\func_Z(x) = 1 - x$.

We suppose that the state of fatigue is not exactly given to us, but we use a probabilistic model in order to estimate it. Suppose the patient performs $H$ sessions and $U$ exercises. At the beginning of each session, the patient is not fatigued, i.e. in state $z_0$. Then, after each exercise, if the patient was in fatigue state $z_i$, he has a probability $p$ of being in the next fatigue state $z_{i+1}$ (until final state of fatigue). At the $i^{th}$ exercise of each session, we can thus easily compute the probability $p_i(z_i)$ of being in state of fatigue $z_i \ \forall i=0,...,Z$. We then assume that the success probability at exercise $i$ is $\sum_{i=0}^Z p_i(z_i)(1 - B_i) f_Z + B_i = (1 - \tilde{B_i}) f_Z + \tilde{B_i}$.

By uniformly sampling difficulties for each exercise of each session, we can then apply Algorithm~\ref{algo-dynamic-setting-general} using contextual features $\tilde{A_i}$ in order to compute the posterior distribution $\tilde{f}(x|\mathcal{S})$. We set parameters $H = 40$, $U = 20$, $Z = 5$ and $p = 0.1$.


==> model.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Model}\label{sec.model}
In the following, we introduce the general problem setting of this paper.
%\paragraph{Space of Bernoulli experiments}  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Space of Bernoulli Experiments}  
Let ($\mathcal{X}, \mathcal{D}$) denote a metric space, where $\mathcal{D}:\mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}_{\geq 0}$ is a distance function. Here, $\mathcal{X}$ could be a continuous set (e.g., $\mathcal{X} = [0, 1]^d$ representing the space of $d$ parameters of a robotic stroke rehabilitation device) or a discrete set (e.g., $\mathcal{X}$  representing different locations in a city). We have a function $\func: \mathcal{X} \rightarrow [0, 1]$ that relates an element of $x \in \mathcal{X}$ to the probability of observing a ``success" outcome when an experiment is performed at $x$. In this paper, our main focus is on learning the function $\func(x)$ for any $x \in \mathcal{X}$ based on a set of Bernoulli experiments, as described below.
% In the application of robotic stroke rehabilitation device, $\func(x)$ relates the probability that a patient will succeed in performing an exercise when the parameters of the device are set to $x$

%let us define $\mathcal{S}(\mathcal{X}, \func)$let us define 
Formally, $(\mathcal{X}, \func)$ defines a space of Bernoulli experiments in our model. A Bernoulli experiment $S_{i}$ is described by the point $x_i \in \mathcal{X}$ at which the experiment is performed, and $s_i \in \{0,1\}$ which denotes the success/failure outcome of the experiment.  We consider two different settings on how we model probability of success of the experiment $S_i$.

\paragraph{Static setting} In a simpler setting, what we call as ``static setting", each experiment is described by a pair $S_i=(x_i, s_i)$ and we model the probability of success as follows:
\begin{align}
Pr(s_{i} = 1) := \func(x_i), \label{eq.exp-outcome-static}
\end{align}
Hence, in the static setting, the static function $\func$ completely characterizes the probability of success of an experiment.

\paragraph{Dynamic setting} In a more generic setting, what we call as ``dynamic setting", each experiment is described by a quadruplet $S_i=(x_i, s_i, A_i, B_i)$ and we model its probability of success as follows:
\begin{align}
Pr(s_{i} = 1) := A_i \func(x_i) + B_i, \label{eq.exp-dynamic}
\end{align}
where $A_i$ and $B_i$ would depend on contextual factors at time $i$, e.g., the level of fatigue of a patient when performing a rehabilitation exercise at time $i$. We restrict $0 \leq B_i \leq 1$, $0 \leq A_i+B_i \leq 1$ in order to ensure that this quantity remains a probability given that $\func(x_i)$ lies in $[0,1]$.  Hence, in the dynamic setting, the probability of success of the experiment depends on the function $\func$ as well as some contextual features dependent on the time $i$. For the case of dynamic setting, we assume that we have knowledge of $A_i$ and $B_i$ (e.g., knowing that how the fatigue state of a patient at a time affects her success probability in an exercise). As we will discuss this further in the theoretical results, we only need to know unbiased estimates of $A_i$ and $B_i$ instead of true values.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Our Objective: Learning $\func$}
%Bernoulli Experiments and Learning Objective
The function $\func$ is unknown and we seek to learn this function from a given set $\mathcal{S} = \{S_{i}\}_{i=1,...,t}$ of $t$ Bernoulli experiments. From these $t$ observations, we want to infer $\func(x)$ for any $x \in \mathcal{X}$.

%For the ease of presentation of our theoretical results, we will consider a batch setting where the set of experiments $\mathcal{S}$ is given to us. For instance, in the rehabilitation application, we have $t$ observations about the patients' success/failure when asked to exercise with different parameters of the device at different time steps $i \in [t]$ (which in turn could be associated with different contextual factors of fatigue state in the dynamic setting).

For each $x \in \mathcal{X}$, we model our belief of the function $\func(x)$ by a random variable $\tilde{\func}(x)$. Our goal is to design an inference engine that can efficiently update our belief $\tilde{\func}(x)$ conditioned on the outputs of the experiments $\mathcal{S}$, denoted as $\tilde{\func}(x|\mathcal{S})$ . In particular, as the size of experiments grow, we would like our belief $\tilde{\func}(x|\mathcal{S})$ to converge to $\func(x)$ at a certain rate, 
\begin{align}
\lim_{t\rightarrow \infty} \mathbb{E}_{\mathcal{S}} \bigg[ \mathbb{E}_{\tilde{\func}}\Big[\big(\tilde{\func}(x|\mathcal{S}) - \func(x)\big)^2\Big] \bigg]= 0, \label{eq.objective}
\end{align}
 where the inner expectation is over the posterior distribution of  $\tilde{\func}(x|\mathcal{S})$ and outer expectation is over the set of experiments and their outcomes, $\mathcal{S}$, due to randomness as to how the experiment points are selected and their outcomes are generated.
 %and outer expectation is over the randomness in the way experiments $\mathcal{S}$  were done and their outcomes.
%\ali{(and outer expectation is over the set of experiments and their outcomes, $\mathcal{S}$, due to randomness as to how the experiment points are selected and their outcomes are generated)}

%%%%%%%%%%%%%
% so that for any $x\in \mathcal{X}$ , we have the following convergence with a certain rate
 %$\tilde{\func}(x|\mathcal{S})$ denotes the posterior distribution of $\tilde{\func}(x)$ based on the experiments $\mathcal{S}$,
%%%%%%%%%%%%%
  
%For each $x \in \mathcal{X}$, we model our knowledge of the probability $\func(x)$ by a random variable $\tilde{\func}(x)$. For both settings, our goal is to design a way of updating our belief $\tilde{\func}(x)$ conditioned on the outputs of the experiments $S$, and on the smoothness assumption for $\func$ so that $\lim_{t\rightarrow \infty} \mathbb{E}_{S,X} \mathbb{E}\left[(\tilde{\func}(x)|S - \func(x))^2\right] = 0$ $\forall x\in \mathcal{X}$ with a certain rate, where $\tilde{\func}(x)|S$ denotes the posterior distribution of $\tilde{\func}(x)$.

%and for each of these experiments, the patient could have a different fatigueness.
 

%Suppose we perform a set of experiments $S = \{S_{x_i}\}_{i=1,...,n}$ at various points of the space $X = \{x_i\}_{i=1,...,n}$. 

%Next, we describe the process of learning $\func$ from a set of Bernoulli experiments. We will consider two settings: (i) a static setting where 

%Formally, let $\mathcal{S}(\mathcal{X}, \func)$ define a space of Bernoulli experiments denoted as $S_x$. Each such experiment $S_x$ is parameterized by $x \in \mathcal{X}$ and the probability of success $Pr(S_x = 1)$ depends on $\func(x)$ and the context . 

%\paragraph{Static setting:} Suppose we perform a set of experiments $S = \{S_{x_i}\}_{i=1,...,n}$ at various points of the space $X = \{x_i\}_{i=1,...,n}$. Each experiment $S_{x_i}$ is an observation of a sample from a Bernoulli random variable with parameter $\func(x_i)$. 

%\paragraph{Dynamic setting:} In a second setting, we suppose that each observation $S_{x_i}$ in the experiments set $S$ is a sample from a Bernoulli random variable with parameter $A_i\func(x_i) + B_i$, where $0 \leq B_i \leq 1$, $0 \leq A_i+B_i \leq 1$ $\forall i$ in order to ensure that this quantity remains a probability whatever the value of $\func(x_i)$ is.


%$\forall i$ 
%as well as any extrinsic features depending on $i$. For instance, in the rehabilitation 

% and $i$ represents the ``time" at which the experiment was performed

%function $f: [\func(x), i, B_i)$ where 

%depends on the function 

%Consider an $i^{\text{th}}$ experiment performed on point $x \in \mathcal{X}$ denoted as $S_{x,i}$. 
%
%$Pr(S_{x,i} = 1)$. The probability of success $Pr(S_{x,i} = 1)$ depends on $\func(x)$ and a time-dependent context at time $i$ given by .

% denoted as $S_x$. Each such experiment $S_x$ is parameterized by $x \in \mathcal{X}$ and the probability of success $Pr(S_x = 1)$ depends on $\func(x)$ and the context . 


%%%%%%%%%%%%%%%%%%%%%%
%In this work for our theoretical results, we will make the following the assumption that the points $x_i$ for $i \in [n]$ experiments are sampled uniformly at random from $\mathcal{X}$
% where $x_i \in \mathcal{X}$ is the point and $s_i \in \{0,1\}$ is the outcome of the $i^{\text{th}}$ experiment. 


%associated with their outcomes $s_i \ \forall i \in [n]$.

%. For each of these experiments $S_{i,x_i}$, we have the success/failure outcome available to us via $s_i$.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experience Sharing and Smoothness Assumption}  
In general, if we make no assumption on the underlying function $\func$, we must perform sufficiently many experiments at every point $x \in \mathcal{X}$ in order to estimate $\func(x) \ \forall x \in \mathcal{X}$. The basic idea to speed up learning and sharing information across experiments is to make some structural assumption on $\func$. For instance, in the robotic stroke rehabilitation framework, it is natural to assume that $\func(x)$ and $\func(x')$ would be correlated with each other if the parameters $x$ and $x'$ are similar. In this paper, we assume that the underlying function $\func$ is ``smooth" and that there exists a constant $L \in \mathbb{R}^+$ such that $|\func(x) - \func(x')| \leq L\mathcal{D}(x,x') \ \forall x, x' \in \mathcal{X}$ (i.e., $\func$ is L-Lipschitz continuous with respect to the distance function $\mathcal{D}$).  

In this paper, we will device an efficient inference engine to leverage this smoothness assumption to speed up learning of $\func$ by sharing the experience of experiments at different points $x \in \mathcal{X}$. Furthermore, we provide convergence rates in $l^2$-norm for both the static and dynamic settings.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%That is, without any additional assumption, there is no way of ``sharing" information across experiments.
%then in order to learn $\func$ at a specific point $x_1 \in \mathcal{X}$ we 


%representing nodes in a graph of different cities of the world 
%representing different concepts in a knowledge graph

%\ali{The language, notations and explanations are very similar to CCBP paper, we may need to revise this section once again}

%Consider a space $\mathcal{S}$  of Bernoulli experiments $S_x$, parametrized by $x \in \mathcal{X}$ with unknown probability of success $\func(x) = Pr(S_x = 1)$.

%We assume that this function $\func$ is smooth in some sense, so that outputs of different experiments $S_x$ and $S_{x'}$ may be correlated. More precisely, let the pair $(S, d)$ denote a metric space, where $d:\mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}^+$ is a distance function. We assume that there exists a constant $L \in \mathbb{R}^+$ such that $|\func(x) - \func(x')| \leq Ld(x,x')$ $\forall x, x' \in \mathcal{X}$ (i.e. $\func$ is L-Lipschitz continuous with respect to distance function $d$).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\ali{The language, notations and explanations are very similar to CCBP paper, we may need to revise this section once again}
%
%Consider a space $\mathcal{S}$  of Bernoulli experiments $S_x$, parametrized by $x \in \mathcal{X}$ with unknown probability of success $\func(x) = Pr(S_x = 1)$. We assume that this function $\func$ is smooth in some sense, so that outputs of different experiments $S_x$ and $S_{x'}$ may be correlated. More precisely, let the pair $(S, d)$ denote a metric space, where $d:\mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}^+$ is a distance function. We assume that there exists a constant $L \in \mathbb{R}^+$ such that $|\func(x) - \func(x')| \leq Ld(x,x')$ $\forall x, x' \in \mathcal{X}$ (i.e. $\func$ is L-Lipschitz continuous with respect to distance function $d$).
%
%\paragraph{Static setting:} Suppose we perform a set of experiments $S = \{S_{x_i}\}_{i=1,...,n}$ at various points of the space $X = \{x_i\}_{i=1,...,n}$. Each experiment $S_{x_i}$ is an observation of a sample from a Bernoulli random variable with parameter $\func(x_i)$. 
%
%\paragraph{Dynamic setting:} In a second setting, we suppose that each observation $S_{x_i}$ in the experiments set $S$ is a sample from a Bernoulli random variable with parameter $A_i\func(x_i) + B_i$, where $0 \leq B_i \leq 1$, $0 \leq A_i+B_i \leq 1$ $\forall i$ in order to ensure that this quantity remains a probability whatever the value of $\func(x_i)$ is.
%
%For each $x \in \mathcal{X}$, we model our knowledge of the probability $\func(x)$ by a random variable $\tilde{\func}(x)$. For both settings, our goal is to design a way of updating our belief $\tilde{\func}(x)$ conditioned on the outputs of the experiments $S$, and on the smoothness assumption for $\func$ so that $\lim_{t\rightarrow \infty} \mathbb{E}_{S,X} \mathbb{E}\left[(\tilde{\func}(x)|S - \func(x))^2\right] = 0$ $\forall x\in \mathcal{X}$ with a certain rate, where $\tilde{\func}(x)|S$ denotes the posterior distribution of $\tilde{\func}(x)$.
